Roadmap to Neuromorphic Computing with Emerging Technologies

The roadmap is organized into several thematic sections, outlining current computing challenges, discussing the neuromorphic computing approach, analyzing mature and currently utilized technologies, providing an overview of emerging technologies, addressing material challenges, exploring novel computing concepts, and finally examining the maturity level of emerging technologies while determining the next essential steps for their advancement.

==> rsriaua78r.tex <==
There are essentially two key properties that make PCM devices particularly well suited for neuromorphic computing (see Figure \ref{163638}) \cite{sebastian2018tutorial}. Interestingly this was pointed out by Stanford Ovshinsky, a pioneer of PCM technology, way back in 2003 when PCM was being considered just for memory applications \cite{ovshinsky2003cognitive}. The first property is that PCM devices can store a range of conductance values by modulating the size of the amorphous region typically achieved by partial RESET pulses that melt and quench a certain volume of PCM material. This analogue storage capability, combined with a crossbar topology, allows for matrix-vector multiply (MVM) operations to be carried out in O(1) time complexity by leveraging Kirchhoff's circuit laws. This makes it possible to realize an artificial neural network on crossbar arrays of PCM devices, with each synaptic layer of the DNN mapped to one or more of the crossbar arrays \cite{Y2017burrAPX,Y2022legalloHERMES}. The second property referred to as accumulative property results from the progressive crystallization of PCM material upon application of an increasing number of partial SET pulses (see Figure 1). It is used for implementing DNN training \cite{Y2020nandakumarFN}, temporal correlation detection \cite{sebastian2017temporal}, continual learning \cite{karunaratne2022memoryContinual}, local learning rules such as spike-timing-dependent plasticity \cite{Y2016ambrogioFN,Y2016tumaEDL} and neuronal dynamics \cite{tuma2016stochasticNeuron}. \\

PCM is at a very high maturity level of development and has been commercialized as both standalone memory\cite{3DXPoint} and embedded memory \cite{Y2020arnaudIEDM}. This fact, together with the ease of embedding PCM on logic platforms (embedded PCM) \cite{Y2022legalloHERMES} make this technology of unique interest for neuromorphic computing.
\subsubsection{5.2.2.Challenges}

PCM devices offer write operations in the tens of nanosecond timescale which is sufficient for most neuromorphic applications in particular those targetting deep learning inference. The cycling endurance could also exceed a billion cycles (dependent on the device geometry) which is several orders of magnitudes higher than commercial Flash memory\cite{lanza2022memristivereview}. This is sufficient for deep learning inference applications. The cycling endurance for partial SET pulses is much higher than that for full SET-RESET cycling and hence is widely considered sufficient for other neuromorphic applications as well. The read endurance is almost infinite for PCM when sufficiently low read bias is applied. Another key attribute is retention which is typically tuned through material choice \cite{Y2009raouxARMR}.  
 However, the use of analogue conductance states in neuromorphic computing makes the retention time of intermediate phase configurations even more important which could be substantially lower than that of fully RESET states.\\
 
One of the primary challenges for PCM is integration density. For example, for DNN inference, it is desirable to have at least 10-100 Million on-chip weight capacity. The crossbar array for neuromorphic computing comprises metal lines intersected by synaptic elements, which are composed of one or more PCM devices and selector devices. Access devices such as bipolar junction transistors or metal-oxide-semiconductor field effect transistors are preferred for accurate programming, while two-terminal poly-silicon diodes offer scalability. To achieve high memory density, stacking multiple crossbar layers vertically is beneficial. BEOL selectors such as ovonic threshold switches show promise but face challenges in achieving precise current control. Edge effects and thermal cross-talk between neighboring cells become significant at smaller feature sizes \cite{LiangEdgeEffect, yoo2020electroThermaldisturbance,lee2010programmingThermaldisturbance}.\\



